Decentralized Control of Partially Observable Markov Decision Processes using Belief Space Macro-actions

The focus of this paper is on solving multi-robot planning problems in continuous spaces with partial observability. Decentralized partially observable Markov decision processes (Dec-POMDPs) are general models for multi-robot coordination problems, but representing and solving Dec-POMDPs is often intractable for large problems. To allow for a high-level representation that is natural for multi-robot problems and scalable to large discrete and continuous problems, this paper extends the Dec-POMDP model to the decentralized partially observable semi-Markov decision process (Dec-POSMDP). The Dec-POSMDP formulation allows asynchronous decision-making by the robots, which is crucial in multi-robot domains. We also present an algorithm for solving this Dec-POSMDP which is much more scalable than previous methods since it can incorporate closed-loop belief space macro-actions in planning. These macro-actions are automatically constructed to produce robust solutions. The proposed method's performance is evaluated on a complex multi-robot package delivery problem under uncertainty, showing that our approach can naturally represent multi-robot problems and provide high-quality solutions for large-scale problems.

==> TemplateFiles/inc.tex <==
\IEEEoverridecommandlockouts \overrideIEEEmargins 
%\pagestyle{plain}

\usepackage{TemplateFiles/fullpage}
\usepackage[ruled,vlined,linesnumbered]{TemplateFiles/algorithm2e}
\usepackage{mathrsfs}
\usepackage{graphicx}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{array}
\usepackage{flafter}
%\usepackage{cite}
\usepackage{subfigure}
\usepackage{verbatim}
%\usepackage{bbm}
\usepackage[usenames]{color}
\usepackage[svgnames]{xcolor}
\usepackage{psfrag}
\usepackage{umoline}
\usepackage{hyperref}
%\usepackage{appendix} %[2009/09/02 v1.2b extra appendix facilities]
\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}	% This is needed for \newtheorem and proof environment.
%\usepackage{natbib} % for citing the papers with auther-year format in parantheses.

\providecommand{\citet}[1]{\citeauthor{#1}\,[\citeyear{#1}]}
\providecommand{\citep}[1]{\cite{#1}}

\newtheorem{thm}{Theorem}
\newtheorem{Def}{Definition}
\newtheorem{Problem}{Problem}
\newtheorem{Lem}{Lemma}
\newtheorem{Cor}{Corollary}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{property}{Property}
\newtheorem{Remark}{Remark}
\newtheorem{exmp}{Example}[section]
%\newenvironment{proof}[1][Proof]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

\newcommand{\TypeOfDoc}{IJRR} % This either can be TR or Conf or IJRR
\newcommand{\FinalFlag}{No} % This either can be No or Accepted

\graphicspath{{./figs/}}

\allowdisplaybreaks[1]

\newcommand{\sXX}[1]{\color{blue}XX S: (#1) XX \color{black}}
%\newcommand{\AXX}[1]{\color{orange} XX #1 XX \color{black}}
\newcommand{\aXX}[1]{\color{purple}XX A: #1 XX\color{black}}
\newcommand{\cXX}[1]{\color{green}XX C: #1 XX\color{black}}

